On Making Emerging Trusted Execution Environments Accessible to Developers

New types of Trusted Execution Environment (TEE) architectures like TrustLite and Intel Software Guard Extensions (SGX) are emerging. They bring new features that can lead to innovative security and privacy solutions. But each new TEE environment comes with its own set of interfaces and programming paradigms, thus raising the barrier for entry for developers who want to make use of these TEEs. In this paper, we motivate the need for realizing standard TEE interfaces on such emerging TEE architectures and show that this exercise is not straightforward. We report on our on-going work in mapping GlobalPlatform standard interfaces to TrustLite and SGX.

==> sections/03.B-virtualization.tex <==
\subsection{Realizing a TEE with Virtualization}


\ifnotabridged{
\subsection{Virtualization}
\label{sec:virtualization}

In their 1974 article ``Formal Requirements for Virtualizable Third Generation Architectures''~\cite{PopekG74} Popek and Goldberg outline the basic requirements of hardware assisted virtualization and the charaterstics that such a machine would exibit. Although hardware virtualization was widely adopted by IBM for their mainframes starting with the 1972 release of the System/370 it was not until 2006 that Intel and AMD independently released hardware support for virtualization with x86 which was targeted at the commodity OS market.

Up until this point virtualization on x86 was achieved either with software virtualization or paravirtualization. With software virtualization the entire virtual system had to be provided by the virtual machine environment. This required complex software capable of binary translation and device emulation in order to support the running of unmodified operating systems. With paravirtualization the Virtual Machine Monitor (VMM), which is responsible for managing the resources of the system, implements an API to allow access to the system resources. This requires that the guest operating systems are modified to call these APIs rather than attempting to invoke privileged commands and operations in their own right.

Although many of the driving forces for supporting hardware virtualization have been performance and efficient sharing of resources, virtualization can also play a crucial role in security. One of the 3 characteristics that Popek and Goldberg define ``the VMM is in complete control of system resources''~\cite{PopekG74} has been made possible in x86 over the past decade by including a number of additions that provide better isolation of the VMM and virtual machines running atop of it.

In the interest of brevity we will choose to look at the security impacts of the Intel x86 virtualization, though the respective names of AMD's offering will be included to allow further investigations by the interested reader.

\textbf{Intel VT-x (AMD-V)}: With the traditional software based virtualization efforts the VMM occupied ring 0~\cite{ProtectionRing} while the guest OS resided in a less privileged ring e.g. ring 1. Because the guest operating system is designed to run in ring 0 this resulted in 2 options for the VMM developers, either the VMM must trap all of the calls to privileged operations or the guest operating system must be modified to work in the higher ring. With the introduction of VT-x, which virtualized the CPU and memory subsystems, came a new privilage level, sometimes referred to as ring -1 but more appropriately VMX. This allowed the guests to remain running at ring 0 thus reducing the complexity of the VMM. This reduced complexity and improved status of the VMM, having a protection level designed specifically for it, results in a more secure configuration.

\textbf{Intel EPT (AMD-RVI)}: The memory management unit (MMU) manages the translation of virtual memory addresses, as seen by the operating system, to physical memory addresses where the actual data resides. When working with a virtualized OS there is an added level of indirection required because what the guest views as physical memory (guest-physical) is actually virtual memory (host-virtual) as allocated by the VMM. This resulted in the guest performing guest-virtual to guest-physical page table translations in software before the hardware page table lookups were performed in the MMU to translate the host-virtual memory to the host-physical addresses. Extended Page Tables (EPT) virtualize the MMU by allowing the guest-physical addresses to be treated almost directly as host-virtual addresses with only a small overhead incurred to create a guest page table mapping in the hardware.

\textbf{Intel VT-d (AMD-Vi)}: Virtualization Technology for Directed I/O allows for the virtualization of interrupts and Direct Memory Access (DMA). By virtualizing the I/O memory mappings, hence the other name the input/output memory management unit (IOMMU)~\cite{IOMMU}, VT-d allows for the guest OS to directly map physical memory to a DMA-capable peripheral device. This was previously not possible as the guest OS's view of what it perceived as physical memory was in fact virtual memory addresses that were provided by the VMM as mentioned above. With the addition of the DMA remapping hardware VT-d allows the direct mapping of the guest OS's DMA requests to the DMA-capable device and it allows access controls to be assigned to each memory mapped region. In addition to enable interesting use cases such as virtual appliances~\cite{VTD} where one guest OS can be given complete control of a peripheral, VT-d can also protect itself and other VMs from accidental or malicious access from a DMA capable device. The attack vector here could be that a driver in a guest OS asks the DMA engine of a device to map a region of physical memory that it would otherwise not have access to, thus enabling it to potentially control the memory of another VM or the VMM itself.

\textbf{Virtual Machine Control Structure (VMSC)}~\cite{VMSC}: To achieve the normal context switch from one VM to another the state of the VM including CPU and memory states need to be stored and restored as the VM is switched out of and back into a running state. Without hardware support when attempting to nest one VMM within another, similar issues occur as with the virtual memory mappings to physical memory mappings mentioned above in that each guest VMM must maintain a software mapping of the VM context states under it. Given that these nestings may be arbitrarily deep there is a significant overhead to such an approach. For this reason Intel introduced hardware support for VMSC. As we shall see in section~\ref{subsec:Realizing a TEE with Virtualization} this allows the inclusion of multiple VMMs, that are created for very niche purposes, to be included into a single system.
}\fi


